Comparative Analysis of Polynomials with Their Computational Costs

In this article, we explore the effectiveness of two polynomial methods in solving non-linear time and space fractional partial differential equations. We first outline the general methodology and then apply it to five distinct experiments. The proposed method, noted for its simplicity, demonstrates a high degree of accuracy. Comparative analysis with existing techniques reveals that our approach yields more precise solutions. The results, presented through graphs and tables, indicate that He's and Daftardar-Jafari polynomials significantly enhance accuracy. Additionally, we provide an in-depth discussion on the computational costs associated with these polynomials. Due to its straightforward implementation, the proposed method can be extended for application to a broader range of problems.

==> ref_cost_paper.tex <==

@article{costRw1,
  author = {Yavuz, M. and Özdemir, N.},
  title = {Analysis of an epidemic spreading model with exponential decay law},
  journal = {Mathematical Sciences and Applications E-Notes},
  volume = {8},
  number = {1},
  year = {2020},
  pages = {142--154}
}

@book{cost7,
  author = {Miller, K.S. and Ross, B.},
  title = {An Introduction to the Fractional Calculus and Fractional Differential Equations},
  publisher = {Wiley},
  year = {1993}
}

@book{cost8,
  editor = {Rudolf, H.},
  title = {Applications of Fractional Calculus in Physics},
  publisher = {World Scientific},
  year = {2000}
}

@book{cost9,
  author = {Podlubny, I.},
  title = {Fractional Differential Equations: An Introduction to Fractional Derivatives, Fractional Differential Equations, to Methods of Their Solution and Some of Their Applications},
  volume = {198},
  publisher = {Elsevier},
  year = {1998}
}

@book{cost6,
  author = {Hilfer, R.},
  title = {Applications of Fractional Calculus in Physics},
  publisher = {Orlando},
  year = {1999}
}

@article{costa1,
  author = {Ubriaco, M.R.},
  title = {Entropies based on fractional calculus},
  journal = {Physics Letters A},
  year = {2009},
  volume = {373},
  pages = {2516--2519}
}

@inproceedings{cost5,
  author = {He, J.H.},
  title = {Nonlinear oscillation with fractional derivative and its applications},
  booktitle = {International Conference on Vibrating Engineering},
  volume = {98},
  pages = {288--291},
  month = {August},
  year = {1998}
}

@article{costt1,
  author = {Zahran, M.A. and El-Shewy, E.K.},
  title = {Contribution of Higher-Order Dispersion to Nonlinear Electron-Acoustic Solitary Waves in a Relativistic Electron Beam Plasma System},
  journal = {Physica Scripta},
  year = {2008},
  volume = {78}
}

@article{costt2,
  author = {Prehl, J. and Essex, C. and Hoffmann, K.H.},
  title = {Tsallis relative entropy and anomalous diffusion},
  journal = {Entropy},
  year = {2012},
  volume = {14},
  pages = {701--716}
}

@article{costt3,
  author = {Sibatov, R. and Shulezhko, V. and Svetukhin, V.},
  title = {Fractional Derivative Phenomenology of Percolative Phonon Assisted Hopping in Two-Dimensional Disordered Systems},
  journal = {Entropy},
  year = {2017},
  volume = {19},
  pages = {463}
}

@article{cost4,
  author = {Longhi, S.},
  title = {Fractional Schrödinger equation in optics},
  journal = {Optics Letters},
  year = {2015},
  volume = {40},
  number = {6},
  pages = {1117--1120}
}

@article{cost2,
  author = {Chaurasia, V.B.L. and Kumar, D.},
  title = {Solution of the time-fractional Navier-Stokes equation},
  journal = {General Mathematics Notes},
  year = {2011},
  volume = {4},
  number = {2},
  pages = {49--59}
}

@article{cost3,
  author = {He, J.H.},
  title = {Homotopy perturbation technique},
  journal = {Computer Methods in Applied Mechanics and Engineering},
  year = {1999},
  volume = {178},
  number = {3-4},
  pages = {257--262}
}
@article{cost1,
  author = {He, J.H.},
  title = {Homotopy perturbation method for solving boundary value problems},
  journal = {Physics Letters A},
  volume = {350},
  number = {1},
  year = {2006},
  pages = {87--88}
}

@article{costhes,
  author = {Ghorbani, A.},
  title = {Beyond Adomian polynomials: he polynomials},
  journal = {Chaos, Solitons \& Fractals},
  volume = {39},
  number = {3},
  year = {2009},
  pages = {1486--1492}
}

@article{cost54,
  author = {Khan, Q. and Khan, H. and Kumam, P. and Tchier, F. and Singh, G.},
  title = {LADM procedure to find the analytical solutions of the nonlinear fractional dynamics of partial integro-differential equations},
  journal = {Demonstratio Mathematica},
  volume = {57},
  number = {1},
  year = {2024},
  pages = {20230101}
}

@article{costr3,
  author = {Dehghan, M. and Abbaszadeh, M.},
  title = {A finite difference/finite element technique with error estimate for space fractional tempered diffusion-wave equation},
  journal = {Computers and Mathematics with Applications},
  volume = {75},
  year = {2018},
  pages = {2903--2914}
}

@article{costr4,
  author = {Yépez-Martínez, H. and Gómez-Aguilar, F. and Sosa, I.O. and Reyes, J.M. and Torres-Jiménez, J.},
  title = {The Feng’s first integral method applied to the nonlinear mKdV space-time fractional partial differential equation},
  journal = {Revista Mexicana de Física},
  volume = {62},
  year = {2016},
  pages = {310--316}
}

@article{costr24,
  author = {Tripathi, N. and Das, S. and Ong, S. and Jafari, H. and Al Qurashi, M.},
  title = {Solution of higher order nonlinear time-fractional reaction diffusion equation},
  journal = {Entropy},
  volume = {18},
  year = {2016},
  pages = {329}
}

@article{costr25,
  author = {Shah, K. and Khalil, H. and Khan, R.A.},
  title = {Analytical solutions of fractional order diffusion equations by natural transform method},
  journal = {Iranian Journal of Science and Technology, Transactions of Science},
  volume = {92},
  year = {2016},
  pages = {1479--1490}
}

@article{costr27,
  author = {Zafarghandi, F.S. and Mohammadi, M. and Babolian, E. and Javadi, S.},
  title = {Radial basis functions method for solving the fractional diffusion equations},
  journal = {Applied Mathematics and Computation},
  volume = {342},
  year = {2019},
  pages = {224--246}
}

@article{costRw2,
  author = {Ojo, G.O. and Mahmudov, N.I.},
  title = {Aboodh transform iterative method for spatial diffusion of a biological population with fractional-order},
  journal = {Mathematics},
  volume = {9},
  number = {2},
  year = {2021},
  pages = {155}
}

@article{costr26,
  author = {Kumar, D. and Singh, J. and Kumar, S.},
  title = {Numerical computation of fractional multi-dimensional diffusion equations by using a modified homotopy perturbation method},
  journal = {Journal of the Association of Arab Universities for Basic and Applied Sciences},
  volume = {17},
  year = {2015},
  pages = {20--26}
}

@article{cost23,
  author = {Ma, W.X. and Zhu, Z.},
  title = {Solving the (3+1)-dimensional generalized KP and BKP equations by the multiple exp-function algorithm},
  journal = {Applied Mathematics and Computation},
  volume = {218},
  number = {24},
  year = {2012},
  pages = {11871--11879}
}

@article{costZ1,
  author = {Phang, C. and Kanwal, A. and Loh, J.R.},
  title = {New collocation scheme for solving fractional partial differential equations},
  journal = {Hacettepe Journal of Mathematics and Statistics},
  volume = {49},
  number = {3},
  year = {2020},
  pages = {1107--1125}
}

@article{costZ2,
  author = {Phang, C. and Toh, Y.T. and Md Nasrudin, F.S.},
  title = {An operational matrix method based on poly-Bernoulli polynomials for solving fractional delay differential equations},
  journal = {Computation},
  volume = {8},
  number = {3},
  year = {2020},
  pages = {82}
}

@article{costvim,
  author = {He, J.H. and Latifizadeh, H.},
  title = {A general numerical algorithm for nonlinear differential equations by the variational iteration method},
  journal = {International Journal of Numerical Methods for Heat and Fluid Flow},
  volume = {30},
  number = {11},
  year = {2020},
  pages = {4797--4810}
}

@article{cost18,
  author = {Young, G. O.},
  title = {Definition of physical consistent damping laws with fractional derivatives},
  journal = {Zeitschrift für Angewandte Mathematik und Mechanik},
  volume = {75},
  year = {1995},
  pages = {623--635}
}

@book{cost11,
  author = {Podlubny, I.},
  title = {Fractional Differential Equations},
  publisher = {Academic Press},
  address = {New York, NY, USA},
  year = {1999}
}

@article{cost12,
  author = {Mainardi, F. and Luchko, Y. and Pagnini, G.},
  title = {The fundamental solution of the space-time fractional diffusion equation},
  journal = {Fractional Calculus and Applied Analysis},
  volume = {4},
  pages = {153--192},
  year = {2001}
}

@article{cost13,
  author = {Debnath, L.},
  title = {Fractional integrals and fractional differential equations in fluid mechanics},
  journal = {Fractional Calculus and Applied Analysis},
  volume = {6},
  pages = {119--155},
  year = {2003}
}

@book{cost14,
  author = {Caputo, M.},
  title = {Elasticita e Dissipazione},
  publisher = {Zani-Chelli},
  address = {Bologna, Italy},
  year = {1969}
}

@book{cost15,
  author = {Miller, K. S. and Ross, B.},
  title = {An Introduction to the Fractional Calculus and Fractional Differential Equations},
  publisher = {Wiley},
  address = {New York, NY, USA},
  year = {1993}
}

@book{cost16,
  author = {Oldham, K. B. and Spanier, J.},
  title = {The Fractional Calculus: Theory and Applications of Differentiation and Integration to Arbitrary Order},
  publisher = {Academic Press},
  address = {New York, NY, USA},
  year = {1974}
}

@book{cost17,
  author = {Kilbas, A. A. and Srivastava, H. M. and Trujillo, J. J.},
  title = {Theory and Applications of Fractional Differential Equations},
  publisher = {Elsevier},
  address = {Amsterdam, The Netherlands},
  year = {2006}
}

@book{costg1,
  author = {Strogatz, S. H.},
  title = {Nonlinear Dynamics and Chaos: With Applications to Physics, Biology, Chemistry, and Engineering},
  publisher = {CRC Press},
  year = {2018}
}

@article{cost105,
  author = {Daftardar-Gejji, V. and Jafari, H.},
  title = {An iterative method for solving nonlinear functional equations},
  journal = {Journal of Mathematical Analysis and Applications},
  volume = {316},
  number = {2},
  pages = {753--763},
  year = {2006}
}

@inproceedings{costDJ2,
  author = {Daftardar-Gejji, V. and Bhalekar, S.},
  title = {An iterative method for solving fractional differential equations},
  booktitle = {PAMM: Proceedings in Applied Mathematics and Mechanics},
  volume = {7},
  number = {1},
  pages = {2050017--2050018},
  year = {2007},
  month = {December},
  publisher = {WILEY-VCH Verlag},
  address = {Berlin}
}

@book{costAD2,
  author = {Adomian, G.},
  title = {Solving Frontier Problems of Physics: The Decomposition Method},
  volume = {60},
  publisher = {Springer Science \& Business Media},
  year = {2013}
}

@article{costAD3,
  author = {Wazwaz, A. M.},
  title = {A new algorithm for calculating Adomian polynomials for nonlinear operators},
  journal = {Applied Mathematics and Computation},
  volume = {111},
  number = {1},
  pages = {33--51},
  year = {2000}
}

@article{costqasim1,
  author = {Khan, Q. and Suen, A. and Khan, H.},
  title = {Application of an efficient analytical technique based on Aboodh transformation to solve linear and non-linear dynamical systems of integro-differential equations},
  journal = {Partial Differential Equations in Applied Mathematics},
  volume = {11},
  pages = {100848},
  year = {2024}
}

@article{costqasim2,
  author = {Khan, Q. and Suen, A. and Khan, H. and Kumam, P.},
  title = {Comparative analysis of fractional dynamical systems with various operators},
  journal = {AIMS Mathematics},
  volume = {8},
  number = {6},
  pages = {13943--13983},
  year = {2023}
}

@article{costqasim3,
  author = {Khan, Q. and Khan, H. and Kumam, P. and Hajira and Sitthithakerngkiet, K.},
  title = {The Fractional Investigation of Some Dynamical Systems With Caputo Operator},
  journal = {Frontiers in Physics},
  volume = {10},
  pages = {895451},
  year = {2022}
}

@article{costqasim4,
  author = {Khan, H. and Kumam, P. and Khan, Q. and Khan, S. and Hajira and Arshad, M. and Sitthithakerngkiet, K.},
  title = {The solution comparison of time-fractional non-linear dynamical systems by using different techniques},
  journal = {Frontiers in Physics},
  volume = {10},
  pages = {863551},
  year = {2022}
}

@article{costqasim5,
  author = {Khan, H. and Khan, Q. and Kumam, P. and Tchier, F. and Singh, G. and Sitthithakerngkiet, K.},
  title = {A modified approach of Adomian decomposition method to solve two-term diffusion wave and time fractional telegraph equations},
  journal = {IEEE Access},
  volume = {10},
  pages = {77475--77486},
  year = {2022}
}

@article{cost43,
  author = {Caputo, M.},
  title = {Linear models of dissipation whose Q is almost frequency independent—II},
  journal = {Geophysical Journal International},
  volume = {13},
  number = {5},
  pages = {529--539},
  year = {1967}
}

@article{costmit39,
  author = {Mittag-Leffler, G.},
  title = {Sur la nouvelle fonction $E_\alpha (x)$},
  journal = {Comptes Rendus de l'Académie des Sciences de Paris},
  volume = {137},
  number = {2},
  pages = {554--558},
  year = {1903},
  month = {October 12}
}

@book{costl1,
  author = {Podlubny, I.},
  title = {Fractional Differential Equations},
  publisher = {Academic Press},
  address = {San Diego},
  year = {1999}
}

@book{costl2,
  author = {Mainardi, F.},
  title = {Fractional Calculus and Waves in Linear Viscoelasticity},
  publisher = {Imperial College Press},
  address = {London},
  year = {2010}
}

@book{costl3,
  author = {Miller, K. and Ross, B.},
  title = {An Introduction to the Fractional Calculus and Fractional Differential Equations},
  publisher = {Wiley},
  address = {New York},
  year = {1993}
}

@incollection{costl4,
  author = {Bagley, R.},
  title = {On the fractional order initial value problem and its engineering applications},
  booktitle = {Fractional Calculus and its Applications},
  editor = {K. Nishimoto},
  publisher = {College of Engineering, Nihon University},
  address = {Tokyo, Japan},
  year = {1990},
  pages = {12--20}
}

@article{costl6,
  author = {Hanna, J. and Rowland, J.},
  title = {Fourier Series, Transforms, and Boundary Value Problems},
  publisher = {John Wiley and Sons, Inc.},
  address = {New York},
  year = {1990}
}

@article{costnex1,
  author = {Singh, A. and Pippal, S.},
  title = {Solution of nonlinear fractional partial differential equations by Shehu transform and Adomian decomposition method (STADM)},
  journal = {International Journal of Mathematics for Industry},
  pages = {2350011},
  year = {2023}
}

@article{costGDTM,
  author = {Momani, S. and Odibat, Z.},
  title = {A novel method for nonlinear fractional partial differential equations: combination of DTM and generalized Taylor's formula},
  journal = {Journal of Computational and Applied Mathematics},
  volume = {220},
  number = {1-2},
  pages = {85--95},
  year = {2008}
}

@article{costADM,
  author = {Odibat, Z. and Momani, S.},
  title = {Numerical methods for nonlinear partial differential equations of fractional order},
  journal = {Applied Mathematical Modelling},
  volume = {32},
  number = {1},
  pages = {28--39},
  year = {2008}
}

@article{costAhmad,
  author = {Ahmad, H. and Farooq, M. and Khan, I. and Nawaz, R. and Fewster-Young, N. and Askar, S.},
  title = {Analysis of nonlinear fractional-order Fisher equation using two reliable techniques},
  journal = {Open Physics},
  volume = {22},
  number = {1},
  pages = {20230185},
  year = {2024}
}

@article{cost51a,
  author = {Yavuz, M. and Ozdemir, N. and Baskonus, H. M.},
  title = {Solutions of partial differential equations using the fractional operator involving Mittag-Leffler kernel},
  journal = {The European Physical Journal Plus},
  volume = {133},
  number = {6},
  pages = {215},
  year = {2018}
}

@article{costf1,
  author = {Patel, Y. and Dhodiya, J. M.},
  title = {Application of differential transform method to solve linear, non-linear reaction convection diffusion and convection diffusion problem},
  journal = {International Journal of Pure and Applied Mathematics},
  volume = {109},
  number = {3},
  pages = {529--538},
  year = {2016}
}

@article{cost2w1,
  author = {Kumar, S. and Rashidi, M. M.},
  title = {New analytical method for gas dynamics equation arising in shock fronts},
  journal = {Computer Physics Communications},
  volume = {185},
  number = {7},
  pages = {1947--1954},
  year = {2014}
}

@article{cost2w2,
  author = {Das, S. and Kumar, R.},
  title = {Approximate analytical solutions of fractional gas dynamic equations},
  journal = {Applied Mathematics and Computation},
  volume = {217},
  number = {24},
  pages = {9905--9915},
  year = {2011}
}

@article{cost2w3,
  author = {Jafari, H. and Alipour, M. and Tajadodi, H.},
  title = {Two-dimensional differential transform method for solving nonlinear partial differential equations},
  journal = {International Journal of Research and Reviews in Applied Sciences},
  volume = {2},
  number = {1},
  pages = {47--52},
  year = {2010}
}

@article{cost2w4,
  author = {Kumar, S. and Kocak, H. and Yıldırım, A.},
  title = {A fractional model of gas dynamics equations and its analytical approximate solution using Laplace transform},
  journal = {Zeitschrift für Naturforschung A},
  volume = {67},
  number = {6-7},
  pages = {389--396},
  year = {2012}
}

@article{cost2w5,
  author = {Nadeem, M. and Ali, M. M.},
  title = {Analytical and Approximate Solutions of the Nonlinear Gas Dynamic Equation Using a Hybrid Approach},
  journal = {Journal of Mathematics},
  volume = {2023},
  number = {1},
  pages = {3136490},
  year = {2023}
}

@article{cost2w6,
  author = {Singh, J. and Kumar, D. and Kılıçman, A.},
  title = {Homotopy perturbation method for fractional gas dynamics equation using Sumudu transform},
  journal = {Abstract and Applied Analysis},
  volume = {2013},
  pages = {934060},
  year = {2013}
}

@article{cost2w7,
  author = {Al-luhaibi, M. S. and Saker, N. A.},
  title = {An analytical treatment to fractional gas dynamics equation},
  journal = {Applied and Computational Mathematics},
  volume = {3},
  number = {6},
  pages = {323--329},
  year = {2014}
}

@inproceedings{cost52a,
  author = {Mohamed-Jawad, A. J. A. and Ozel, C. and Kilicman, A.},
  title = {Variational iteration method in solving evolution equations},
  booktitle = {AIP Conference Proceedings},
  volume = {1309},
  number = {1},
  pages = {510},
  year = {2010},
  month = {November}
}

@article{cost52b,
  author = {Jafari, H. and Zabihi, M. and Saidy, M.},
  title = {Application of homotopy perturbation method for solving gas dynamics equation},
  journal = {Applied Mathematical Sciences},
  volume = {2},
  number = {48},
  pages = {2393--2396},
  year = {2008}
}

@article{costHPM,
  author = {Momani, S. and Odibat, Z.},
  title = {Homotopy perturbation method for nonlinear partial differential equations of fractional order},
  journal = {Physics Letters A},
  volume = {365},
  number = {5-6},
  pages = {345--350},
  year = {2007}
}

@article{costRasool,
  author = {Iqbal, N. and Akgül, A. and Shah, R. and Bariq, A. and Mossa Al-Sawalha, M. and Ali, A.},
  title = {On Solutions of Fractional-Order Gas Dynamics Equation by Effective Techniques},
  journal = {Journal of Function Spaces},
  volume = {2022},
  number = {1},
  pages = {3341754},
  year = {2022}
}

@article{costrashid,
  author = {Khalil, M. M. and Rehman, S. U. and Ali, A. H. and Nawaz, R. and Batiha, B.},
  title = {New modifications of natural transform iterative method and q-homotopy analysis method applied to fractional order KDV-Burger and Sawada-Kotera equations},
  journal = {Partial Differential Equations in Applied Mathematics},
  pages = {100950},
  year = {2024}
}




%%%\bibitem{costRw1}
%%%   Yavuz, M. and Özdemir, N., 2020. Analysis of an epidemic spreading model with exponential decay law. Mathematical Sciences and Applications E-Notes, 8(1), pp.142-154.
%%%\bibitem{cost7}
%%%Miller, K.S. and Ross, B., 1993. An introduction to the fractional calculus and fractional differential equations. Wiley.
%%%\bibitem{cost8}
%%%Rudolf, H. ed., 2000. Applications of fractional calculus in physics. world scientific.
%%%\bibitem{cost9}
%%% Podlubny, I., 1998. Fractional differential equations: an introduction to fractional derivatives, fractional differential equations, to methods of their solution and some of their applications (Vol. 198). Elsevier.
%%%\bibitem{cost6}
%%%    Hilfer, R., 1999. Applications of Fractional Calculus in Physics. Orlando.
%%%\bibitem{costa1}
%%%   Ubriaco, M.R. Entropies based on fractional calculus. Phys. Lett. A 2009, 373, 2516-2519
%%%\bibitem{cost5}
%%%    He, J.H., 1998, August. Nonlinear oscillation with fractional derivative and its applications. In International conference on vibrating engineering (Vol. 98, pp. 288-291).
%%%\bibitem{costt1}
%%%    Zahran, M.A.; El-Shewy, E.K. Contribution of Higher-Order Dispersion to Nonlinear Electron-Acoustic Solitary Waves in a Relativistic Electron Beam Plasma System. Phys. Scr. 2008, 78.
%%%\bibitem{costt2}
%%%    Prehl, J.; Essex, C.; Hoffmann, K.H. Tsallis relative entropy and anomalous diffusion. Entropy 2012 , 14, 701-716.
%%%\bibitem{costt3}
%%%   Sibatov, R.; Shulezhko, V.; Svetukhin, V. Fractional Derivative Phenomenology of Percolative Phonon Assisted Hopping in Two-Dimensional Disordered Systems. Entropy 2017, 19, 463.
%%%\bibitem{cost4}
%%%    Longhi, S., 2015. Fractional Schr\"{o}dinger equation in optics. Optics letters, 40(6), pp.1117-1120.
%%%\bibitem{cost2}
%%%   Chaurasia, V.B.L. and Kumar, D., 2011. Solution of the time-fractional Navier-Stokes equation. Gen. Math. Notes,4(2), pp.49-59.
%%%\bibitem{cost3}
%%%   He, J.H., 1999. Homotopy perturbation technique. Computer methods in applied mechanics and engineering, 178(3-4), pp.257-262.
%%%\bibitem{cost1}
%%%    He, J.H., 2006, Homotopy perturbation method for solving boundary value problems. Phys. Lett. A 350(1),87-88
%%%\bibitem{costhes}
%%%   Ghorbani, A., 2009. Beyond Adomian polynomials: he polynomials. Chaos, Solitons \& Fractals, 39(3), pp.1486-1492.
%%%\bibitem{cost54} Khan, Q., Khan, H., Kumam, P., Tchier, F. and Singh, G., 2024. LADM procedure to find the analytical solutions of the nonlinear fractional dynamics of partial integro-differential equations. Demonstratio Mathematica, 57(1), p.20230101.
%%%\bibitem{costr3} Dehghan, M.; Abbaszadeh, M. A finite difference/finite element technique with error estimate for space
%%%   fractional tempered diffusion-wave equation. Comput. Math. Appl. 2018, 75, 2903-2914.
%%%\bibitem{costr4}
%%%    Yépez-Martínez, H.; Gómez-Aguilar, F.; Sosa, I.O.; Reyes, J.M.; Torres-Jiménez, J. The Feng’s first integral
%%%   method applied to the nonlinear mKdV space-time fractional partial differential equation. Rev. Mex. Fís.   2016, 62, 310-316.
%%%\bibitem{costr24}
%%%   Tripathi, N.; Das, S.; Ong, S.; Jafari, H.; Al Qurashi, M. Solution of higher order nonlinear time-fractional
%%%   reaction diffusion equation. Entropy 2016, 18, 329.
%%%\bibitem{costr25}
%%%   Shah, K.; Khalil, H.; Khan, R.A. Analytical solutions of fractional order diffusion equations by natural
%%%   transform method. Iran. J. Sci. Technol. Trans. Sci. 2016, 92, 1479-1490.
%%%\bibitem{costr27}Zafarghandi, F.S.; Mohammadi, M.; Babolian, E.; Javadi, S. Radial basis functions method for solving the
%%%   fractional diffusion equations. Appl. Math. Comput. 2019, 342, 224-246.
%%%\bibitem{costRw2}
%%%    Ojo, G.O. and Mahmudov, N.I., 2021. Aboodh transform iterative method for spatial diffusion of a biological population with fractional-order. Mathematics, 9(2), p.155.
%%%\bibitem{costr26}
%%%   Kumar, D.; Singh, J.; Kumar, S. Numerical computation of fractional multi-dimensional diffusion equations by using a modified homotopy perturbation method. J. Assoc. Arab. Univ. Basic Appl. Sci. 2015, 17, 20-26.
%%%\bibitem{cost23} Ma, W.X. and Zhu, Z., 2012. Solving the (3+ 1)-dimensional generalized KP and BKP equations by the multiple exp-function algorithm. Applied Mathematics and Computation, 218(24), pp.11871-11879.
%%%\bibitem{costZ1}
%%%   Phang, C., Kanwal, A. and Loh, J.R., 2020. New collocation scheme for solving fractional partial differential equations. Hacettepe Journal of Mathematics and Statistics, 49(3), pp.1107-1125.
%%%\bibitem{costZ2}
%%%   Phang, C., Toh, Y.T. and Md Nasrudin, F.S., 2020. An operational matrix method based on poly-Bernoulli polynomials for solving fractional delay differential equations. Computation, 8(3), p.82.
%%%\bibitem{costvim}
%%%   He, J.H. and Latifizadeh, H., 2020. A general numerical algorithm for nonlinear differential equations by the variational iteration method. International Journal of Numerical Methods for Heat \& Fluid Flow, 30(11), pp.4797-4810.
%%%\bibitem{cost18}
%%%G. O. Young, “Definition of physical consistent damping laws
%%%   with fractional derivatives,” Zeitschrift f\"{u}r Angewandte Mathematik
%%%   und Mechanik, vol. 75, pp. 623-635, 1995.
%%%
%%%\bibitem{cost11} I. Podlubny, Fractional Differential Equations, Academic Press,
%%%   New York, NY, USA, 1999.
%%%\bibitem{cost12}
%%% F.Mainardi, Y. Luchko, and G. Pagnini, “The fundamental solution
%%%   of the space-time fractional diffusion equation,” Fractional
%%%   Calculus and Applied Analysis, vol. 4, pp. 153-192, 2001.
%%%\bibitem{cost13}
%%%L. Debnath, “Fractional integrals and fractional differential
%%%   equations in fluid mechanics,” Fractional Calculus and Applied
%%%   Analysis, vol. 6, pp. 119-155, 2003.
%%%\bibitem{cost14}
%%%M. Caputo, Elasticita e Dissipazione, Zani-Chelli, Bologna, Italy,
%%%   1969.
%%%\bibitem{cost15} K. S. Miller and B. Ross, An Introduction to the Fractional
%%%   CalculusandFractionalDifferentialEquations,Wiley,NewYork,
%%%   NY, USA, 1993.
%%%\bibitem{cost16} K. B. Oldham and J. Spanier, The Fractional Calculus Theory
%%%   and Applications of Differentiation and Integration to Arbitrary
%%%   Order, Academic Press, New York, NY, USA, 1974.
%%%\bibitem{cost17} A. A. Kilbas, H. M. Srivastava, and J. J. Trujillo, Theory
%%%   and Applications of Fractional Differential Equations, Elsevier,
%%%   Amsterdam, The Netherlands, 2006.
%%%\bibitem{costg1}
%%%    Strogatz, S.H., 2018. Nonlinear dynamics and chaos: with applications to physics, biology, chemistry, and engineering. CRC press.
%%%\bibitem{cost105}
%%%   Daftardar-Gejji, V. and Jafari, H., 2006. An iterative method for solving nonlinear functional equations. Journal of Mathematical Analysis and Applications, 316(2), pp.753-763.
%%%
%%%\bibitem{costDJ2}
%%%   Daftardar‐Gejji, V. and Bhalekar, S., 2007, December. An iterative method for solving fractional differential equations. In PAMM: Proceedings in Applied Mathematics and Mechanics (Vol. 7, No. 1, pp. 2050017-2050018). Berlin: WILEY‐VCH Verlag.
%%%\bibitem{costAD2}
%%%   Adomian, G., 2013. Solving frontier problems of physics: the decomposition method (Vol. 60). Springer Science \& Business Media.
%%%\bibitem{costAD3}
%%%   Wazwaz, A.M., 2000. A new algorithm for calculating Adomian polynomials for nonlinear operators. Applied Mathematics and computation, 111(1), pp.33-51.
%%%\bibitem{costqasim1}
%%%   Khan, Q., Suen, A. and Khan, H., 2024. Application of an efficient analytical technique based on Aboodh transformation to solve linear and non-linear dynamical systems of integro-differential equations. Partial Differential Equations in Applied Mathematics, 11, p.100848.
%%%\bibitem{costqasim2}
%%%   Khan, Q., Suen, A., Khan, H. and Kumam, P., 2023. Comparative analysis of fractional dynamical systems with various operators. AIMS Mathematics, 8(6), pp.13943-13983.
%%%\bibitem{costqasim3}
%%%   Khan, Q., Khan, H., Kumam, P., Hajira and Sitthithakerngkiet, K., 2022. The Fractional Investigation of Some Dynamical Systems With Caputo Operator. Frontiers in Physics, 10, p.895451.
%%%\bibitem{costqasim4}
%%%   Khan, H., Kumam, P., Khan, Q., Khan, S., Hajira, Arshad, M. and Sitthithakerngkiet, K., 2022. The solution comparison of time-fractional non-linear dynamical systems by using different techniques. Frontiers in Physics, 10, p.863551.
%%%\bibitem{costqasim5}
%%%   Khan, H., Khan, Q., Kumam, P., Tchier, F., Singh, G. and Sitthithakerngkiet, K., 2022. A modified approach of Adomian decomposition method to solve two-term diffusion wave and time fractional telegraph equations. IEEE Access, 10, pp.77475-77486.
%%%
%%%\bibitem{cost43} Caputo, M., 1967. Linear models of dissipation whose Q is almost frequency independent—II. Geophysical journal international, 13(5), pp.529-539.
%%%
%%%\bibitem{costmit39} Mittag-Leffler GM. Sur la nouvelle fonction $E_\alpha (x)$. { \it CR Acad. Sci. Paris. } 1903 Oct 12;137(2):554-8.
%%%\bibitem{costl1}
%%%   Podlubny I. Fractional Differential Equations . Academic Press, San Diego; 1999.
%%%\bibitem{costl2}
%%%   Mainardi F. Fractional Calculus and Waves in Linear Viscoelasticity . Imperial College Press, London; 2010.
%%%\bibitem{costl3}
%%%   Miller K, Ross B. An Introduction to the Fractional Calculus and Fractional Differential Equations . Wiley, New York; 1993.
%%%\bibitem{costl4}
%%%   Bagley R. On the fractional order initial value problem and its engineering applications. In: Fractional Calculus and its Applications . K. Nishimoto, Ed., College of Engineering, Nihon University, Tokyo, Japan; 1990: 12-20.
%%%
%%%\bibitem{costl6}
%%%   Hanna J, Rowland J. Fourier Series, Transforms, and Boundary Value Problems . John Wiley and Sons, Inc., New York; 1990.
%%%\bibitem{costnex1}
%%%   Singh, A. and Pippal, S., 2023. Solution of nonlinear fractional partial differential equations by Shehu transform and Adomian decomposition method (STADM). International Journal of Mathematics for Industry, p.2350011.
%%%\bibitem{costGDTM}
%%%   Momani, S. and Odibat, Z., 2008. A novel method for nonlinear fractional partial differential equations: combination of DTM and generalized Taylor's formula. Journal of Computational and Applied Mathematics, 220(1-2), pp.85-95.
%%%\bibitem{costADM} Odibat, Z. and Momani, S., 2008. Numerical methods for nonlinear partial differential equations of fractional order. Applied Mathematical Modelling, 32(1), pp.28-39.
%%%\bibitem{costAhmad}
%%%    Ahmad, H., Farooq, M., Khan, I., Nawaz, R., Fewster-Young, N. and Askar, S., 2024. Analysis of nonlinear fractional-order Fisher equation using two reliable techniques. Open Physics, 22(1), p.20230185.
%%%
%%%\bibitem{cost51a}
%%%   Yavuz, M., Ozdemir, N. and Baskonus, H.M., 2018. Solutions of partial differential equations using the fractional operator involving Mittag-Leffler kernel. The European Physical Journal Plus, 133(6), p.215.
%%%
%%%\bibitem{costf1}
%%%    Patel, Y. and Dhodiya, J.M., 2016. Application of differential transform method to solve linear, non-linear reaction convection diffusion and convection diffusion problem. International Journal of Pure and Applied Mathematics, 109(3), pp.529-538.
%%%
%%%\bibitem{cost2w1}
%%%   Kumar, S. and Rashidi, M.M., 2014. New analytical method for gas dynamics equation arising in shock fronts. Computer Physics Communications, 185(7), pp.1947-1954.
%%%\bibitem{cost2w2}
%%%   Das, S. and Kumar, R., 2011. Approximate analytical solutions of fractional gas dynamic equations. Applied Mathematics and Computation, 217(24), pp.9905-9915.
%%%\bibitem{cost2w3}
%%%   Jafari, H., Alipour, M. and Tajadodi, H., 2010. Two-dimensional differential transform method for solving nonlinear partial differential equations. International Journal of Research and Reviews in Applied Sciences, 2(1), pp.47-52.
%%%\bibitem{cost2w4}
%%%   Kumar, S., Kocak, H. and Yıldırım, A., 2012. A fractional model of gas dynamics equations and its analytical approximate solution using Laplace transform. Zeitschrift f\"{u}r Naturforschung A, 67(6-7), pp.389-396.
%%%\bibitem{cost2w5}
%%%   Nadeem, M. and Ali, M.M., 2023. Analytical and Approximate Solutions of the Nonlinear Gas Dynamic Equation Using a Hybrid Approach. Journal of Mathematics, 2023(1), p.3136490.
%%%\bibitem{cost2w6}
%%%   Singh, J., Kumar, D. and Kılıçman, A., 2013. Homotopy perturbation method for fractional gas dynamics equation using Sumudu transform. In Abstract and Applied Analysis (Vol. 2013, No. 1, p. 934060). Hindawi Publishing Corporation.
%%%\bibitem{cost2w7}
%%%   Al-luhaibi, M.S. and Saker, N.A., 2014. An analytical treatment to fractional gas dynamics equation. Applied and Computational Mathematics, 3(6), pp.323-329.
%%%\bibitem{cost52a}
%%%    Mohamed-Jawad, A.J.A., Ozel, C. and Kilicman, A., 2010, November. Variational iteration method in solving evolution equations. In Aip Conference Proceedings (Vol. 1309, No. 1, p. 510).
%%%\bibitem{cost52b}
%%%   Jafari, H., Zabihi, M. and Saidy, M., 2008. Application of homotopy perturbation method for solving gas dynamics equation. Applied Mathematical Sciences, 2(48), pp.2393-2396.
%%%\bibitem{costHPM}
%%%   Momani, S. and Odibat, Z., 2007. Homotopy perturbation method for nonlinear partial differential equations of fractional order. Physics Letters A, 365(5-6), pp.345-350.
%%%\bibitem{costRasool}
%%%    Iqbal, N., Akgül, A., Shah, R., Bariq, A., Mossa Al-Sawalha, M. and Ali, A., 2022. On Solutions of Fractional‐Order Gas Dynamics Equation by Effective Techniques. Journal of Function Spaces, 2022(1), p.3341754.
%%%\bibitem{costrashid}
%%%   Khalil, M.M., Rehman, S.U., Ali, A.H., Nawaz, R. and Batiha, B., 2024. New modifications of natural transform iterative method and q-homotopy analysis method applied to fractional order KDV-Burger and Sawada-Kotera equations. Partial Differential Equations in Applied Mathematics, p.100950.
%%%%\end{thebibliography}

